Decentralized utility- and locality-aware replication for heterogeneous DHT-based P2P cloud storage systems

As a Distributed Hash Table (DHT), Skip Graph routing overlays are exploited in several peer-to-peer (P2P) services, including P2P cloud storage. The fully decentralized replication algorithms that are applicable to the Skip Graph-based P2P cloud storage fail on improving the performance of the system with respect to both the availability of replicas as well as their response time. Additionally, they presume the system as homogeneous with respect to the nodes' latency distribution, availability behavior, bandwidth, or storage. In this paper, we propose Pyramid, which is the first fully decentralized utility- and locality-aware replication approach for Skip Graph-based P2P cloud storage systems. Pyramid considers the nodes as heterogeneous with respect to their latency distribution, availability behavior, bandwidth, and storage. Pyramid is utility-aware as it maximizes the average available bandwidth of replicas per time slot (e.g., per hour). Additionally, Pyramid is locality-aware as it minimizes the average latency between nodes and their closest replica. Our simulation results show that compared to the state-of-the-art solutions that either perform good in utility-awareness, or in locality-awareness, our proposed Pyramid improves both the utility- and locality-awareness of replicas with a gain of about 1.2 and 1.1 times at the same time, respectively.

==> Sections/Biography.tex <==
\vskip -3\baselineskip plus -1fil
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Yahya}}]{Yahya Hassanzadeh-Nazarabadi} received the B.S. degree in computer hardware engineering from Ferdowsi University, Mashhad, Iran, in 2013, and the Ph.D. degree in computer science and engineering from Koç University, Istanbul, Turkey, in 2019. His research interests are distributed cloud storage systems, blockchains, and security.
\end{IEEEbiography}
\vskip -3\baselineskip plus -1fil
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/AlptekinKupcu-100x125}}]{Alptekin Küpçü} received his Ph.D. degree from Brown University Computer Science Department in 2010. Since then, he has been working as a faculty at Koç University, and leading the Cryptography, Security \& Privacy Research Group he has founded. Dr. Küpçü has various accomplishments including 5 international patents granted, 10 funded research projects (for 8 of which he was the principal investigator), 2 European Union COST Action management committee memberships, 4 Koç University Teaching Awards, 2 Outstanding Young Scientist Awards (BAGEP \& GEBİP), ACM and IEEE Senior Member Awards, and the Royal Society of UK Newton Advanced Fellowship. For more information, visit https://crypto.ku.edu.tr
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/OznurOzkasap}}]{Öznur Özkasap} received the Ph.D. degree in Computer Engineering from Ege University in 2000. From 1997 to 1999, she was a Graduate Research Assistant with the Department of Computer Science, Cornell University, where she completed her Ph.D. dissertation. She is currently a Professor with the Department of Computer Engineering, Koç University, which she joined in 2000. Her research interests include distributed systems, multicast protocols, peer-to-peer systems, bio-inspired distributed algorithms, mobile and vehicular ad hoc networks, energy efficiency, cloud computing, and computer networks. Dr. Özkasap serves as an Area Editor of the Future Generation Computer Systems journal, Elsevier Science, and National Representative of ACM-W Europe. She is a recipient of the Turk Telekom Collaborative Research Awards, the Career Award of TUBITAK (The Scientific and Technological Research Council of Turkey), and TUBITAK/NATO A2 Ph.D. Research Scholarship Abroad, and she was awarded Teaching Innovation Grants by Koç University.

\end{IEEEbiography}
